Learning Easily Updated General Purpose Text Representations with Adaptable Task-Specific Prefixes

Many real-world applications require making multiple predictions from the same text. Fine-tuning a large pre-trained language model for each downstream task causes computational burdens in the inference time due to several times of forward passes. To amortize the computational cost, freezing the language model and building lightweight models for downstream tasks based on fixed text representations are common solutions. Accordingly, how to learn fixed but general text representations that can generalize well to unseen downstream tasks becomes a challenge. Previous works have shown that the generalizability of representations can be improved by fine-tuning the pre-trained language model with some source tasks in a multi-tasking way. In this work, we propose a prefix-based method to learn the fixed text representations with source tasks. We learn a task-specific prefix for each source task independently and combine them to get the final representations. Our experimental results show that prefix-based training performs better than multi-tasking training and can update the text representations at a smaller computational cost than multi-tasking training.

==> 91-Tasks.tex <==
\section{Tasks}
\label{app:tasks}

We consider different types of NLP tasks, including natural language inference, paraphrase identification, sentiment analysis, question answering, commonsense reasoning, as listed in Table~\ref{tab:data}.
The source tasks include the following 7 datasets with more than 40K annotations:
MNLI \cite{Williams18mnli}, QNLI \cite{Demszky18qnli}, QQP \cite{Wang19glue}, SST-2 \cite{Socher13sst2}, Yelp-2 \cite{Charwad17yelp2}, ReCoRD \cite{Zhang18record}, and WinoGrande \cite{Sakaguchi20winogrande}.
The target tasks include the following 8 datasets:
RTE \cite{Giampiccolo07rte}, MRPC \cite{Dolan04mrpc}, CR \cite{Hu04cr}, MR \cite{Pang05mr}, MPQA \cite{Wiebe05mpqa}, BoolQ \cite{Clark19boolq}, MultiRC \cite{Khashabi18multirc}, and CosmosQA \cite{Huang19cosmosqa}.

For those datasets with the standard train/dev/test split, we use the standard split for training.
For those datasets without the standard train/dev/test split (e.g., GLUE tasks), we randomly split 1/3 examples from the dev set as the internal dev set and use the rest 2/3 examples as the testing set.

\begin{table}[t!]
\small
\centering
\setlength{\tabcolsep}{4pt}
\resizebox{.48\textwidth}{!}{
\begin{tabular}{llr}
    \toprule
    Dataset & Task Type & \# of Train \\
    \midrule
    \multicolumn{3}{l}{\emph{Source Tasks}} \\
    \midrule
    MNLI       & Natural Language Inference (NLI) & 393K \\
    QNLI       & Natural Language Inference	(NLI) & 105K \\
    QQP        & Paraphrase Identification (PI)   & 364K \\
    SST-2      & Sentiment Analysis	(SA)          &  66K \\
    Yelp-2     & Sentiment Analysis	(SA)          & 540K \\
    ReCoRD     & Question Answering (QA)          & 101K \\
    WinoGrande & Commonsense Reasoning (CR)       &  40K \\
    \midrule
    \multicolumn{3}{l}{\emph{Target Tasks}} \\
    \midrule
    RTE        & Natural Language Inference	(NLI) & 2.5K \\
    MRPC       & Paraphrase Identification (PI)   & 3.7K \\
    CR         & Sentiment Analysis (SA)          & 2.3K \\
    MR         & Sentiment Analysis (SA)          & 6.4K \\
    MPQA       & Sentiment Analysis (SA)          & 6.4K \\
    BoolQ      & Question Answering (QA)          & 9.4K \\
    MultiRC    & Question Answering (QA)          &  27K \\
    CosmosQA   & Commonsense Reasoning (CR)       &  25K \\
    \bottomrule
\end{tabular}}
\caption{Datasets.}
\label{tab:data}
\end{table}

